Galactic positrons and electrons from astrophysical sources and dark matter

A very interesting puzzle about the origin of electron and positron cosmic rays is deduced from the latests experimental results. We model the propagation of such cosmic rays in terms of a successfully tested two--zone propagation model. Several theoretical uncertainties -- like ones related to propagation -- are considered to study different types of electron and positron sources: dark matter annihilation, secondary production, and supernova remnants.

==> tex/discu.tex <==
\section{Discussion}
\label{sec4}

